Snoopy: A Webpage Fingerprinting Framework with Finite Query Model for Mass-Surveillance

Internet users are vulnerable to privacy attacks despite the use of encryption. Webpage fingerprinting, an attack that analyzes encrypted traffic, can identify the webpages visited by a user in a given website. Recent research works have been successful in demonstrating webpage fingerprinting attacks on individual users, but have been unsuccessful in extending their attack for mass-surveillance. The key challenges in performing mass-scale webpage fingerprinting arises from (i) the sheer number of combinations of user behavior and preferences to account for, and; (ii) the bound on the number of website queries imposed by the defense mechanisms (e.g., DDoS defense) deployed at the website. These constraints preclude the use of conventional data-intensive ML-based techniques. In this work, we propose Snoopy, a first-of-its-kind framework, that performs webpage fingerprinting for a large number of users visiting a website. Snoopy caters to the generalization requirements of mass-surveillance while complying with a bound on the number of website accesses (finite query model) for traffic sample collection. For this, Snoopy uses a feature (i.e., sequence of encrypted resource sizes) that is either unaffected or predictably affected by different browsing contexts (OS, browser, caching, cookie settings). Snoopy uses static analysis techniques to predict the variations caused by factors such as header sizes, MTU, and User Agent String that arise from the diversity in browsing contexts. We show that Snoopy achieves approximately 90% accuracy when evaluated on most websites, across various browsing contexts. A simple ensemble of Snoopy and an ML-based technique achieves approximately 97% accuracy while adhering to the finite query model, in cases when Snoopy alone does not perform well.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> backup.tex <==
\subsection{Snoopy-ML Ensemble}\label{sec:snoopy-meets-ml}
Our studies and experiments so far show that Snoopy and known ML-based techniques have some distinct advantages and disadvantages. While Snoopy offers a generalized prediction framework while complying with a finite query model (refer to Section~\ref{results}), it is restricted by the low number of stable features available for webpage classification. Therefore, Snoopy fails to predict webpages whose the resource sizes and resource download sequences are similar to those of other webpages in the website (Refer to Section~\ref{sec:resvspage}). On the other hand, ML-based techniques use a plethora of features to classify webpages with high accuracy. While these techniques are very useful for classifying a small number of webpages (targeted surveillance), we have seen that they cannot be scaled for building the generalized framework that mass-surveillance requires (refer to Section~\ref{results}). This is because the huge number of traffic samples that would be required for building a generalized ML-based prediction framework would defy our finite query model. In this section, we explore the following question: {\em``Can we can combine the complementary advantages provided by Snoopy and ML to build an ensemble prediction framework that enhances the overall webpage prediction accuracy, while complying with a finite query model?"}   

Figure~\ref{fig:ensemble-training} shows how Snoopy and ML-based techniques are combined to build an ensemble prediction model. The fundamental idea behind building the ensemble model is that we use ML-based techniques only for classifying those webpages that Snoopy fails to classify accurately. Since the fraction of such webpages is low as compared to the total number of webpages in a website (on an average $\approx10\%$ for the websites we considered), ML-based techniques can classify them with a high accuracy even with a comparatively small number of traffic samples. This makes the ensemble model compliant with a finite query model. Training the ensemble model for a targeted website involves the following two steps.

\noindent\textbf{(Step 1)} Once the traffic samples are collected for Snoopy, the $n$ samples for each of the webpages (comprising the set of all webpages $\mathbb{W}$) are divided into two parts -- one for webpage profiling, and the other part for validation of the Snoopy framework. Using the first part, the Webpage Profiling Module of Snoopy extracts the resource signatures and other metadata required for webpage prediction. Next, the other half of traffic samples are passed to the Prediction Module of Snoopy in encrypted form and the prediction accuracy for each webpage is noted. The output of this step is the set of webpages $\mathbb{W}_1$ that Snoopy is unable to identify accurately.

\noindent\textbf{(Step 2)} In this step, we first collect more traffic samples (say, $n_1$) for each webpage in $\mathbb{W}_1$, if required, to account for all the generalization factors that the adversary is interested in. Next, an ML-based technique is used to model the encrypted traffic characteristics of the webpages in $\mathbb{W}_1$. Similar to all conventional ML-based techniques, this ML model is also validated using a fraction of the traffic samples collected for each webpage. The output of this step is the ML model and the minimum prediction probability (denoted as $P_v$) derived during the validation step. 

Figure~\ref{fig:ensemble-testing} shows how the ensemble model is used for predicting the webpages accessed in an encrypted traffic trace $T$.  
